ADMM Algorithm for Graphical Lasso with an $\ell_{\infty}$ Element-wise Norm Constraint

We consider the problem of Graphical lasso with an additional $\ell_{\infty}$ element-wise norm constraint on the precision matrix. This problem has applications in high-dimensional covariance decomposition such as in \citep{Janzamin-12}. We propose an ADMM algorithm to solve this problem. We also use a continuation strategy on the penalty parameter to have a fast implemenation of the algorithm.

==> macros/macro_JMLR.tex <==

%\newcommand{\reals}{\mathbb{R}}
%\newcommand{\naturals}{\mathbb{N}}

%%%%% ---- MY MACROS ------- %%%%%



%% ------ Equations and Equation arrays ------ %%
\newcommand{\beq}{\begin{eqnarray}}
\newcommand{\eeq}{\end{eqnarray}}
\newcommand{\beqs}{\begin{eqnarray*}}
\newcommand{\eeqs}{\end{eqnarray*}}
\newcommand{\barr}{\begin{array}}
\newcommand{\earr}{\end{array}}
\newcommand{\beqa}{\begin{eqnarray} \begin{array}}
\newcommand{\eeqa}{\end{array} \end{eqnarray}}
\newcommand{\beqas}{\begin{eqnarray*} \begin{array}}
\newcommand{\eeqas}{\end{array} \end{eqnarray*}}

\newcommand{\meq}{&=&}
\newcommand{\mle}{&\leq&}
\newcommand{\mge}{&\geq&}


%% ------ Theorems and lefmmas ---------- %%

\newcommand{\bthm}{\begin{theo}}
\newcommand{\ethm}{\end{theo}}
\newcommand{\blem}{\begin{lem}}
\newcommand{\elem}{\end{lem}}
\newcommand{\bdefn}{\begin{defn}}
\newcommand{\edefn}{\end{defn}}
%\newcommand{\bprf}{\begin{proof}}
%\newcommand{\eprf}{\end{proof}}

\newcommand{\lbeq}[1]{\label{eq:#1}}
\newcommand{\lbth}[1]{\label{theo:#1}}
\newcommand{\lblem}[1]{\label{lem:#1}}
\newcommand{\lbdef}[1]{\label{def:#1}}
%\newcommand{\refeq}[1]{\ref{eq:#1}}
\newcommand{\refthm}[1]{\ref{thm:#1}}
%\newcommand{\refeq}[1]{\ref{eq:#1}}
\newcommand{\refdef}[1]{\ref{def:#1}}


%% ------ Mathematical expressions ------- %%

\newcommand{\sq}{\sqrt}
%\newcommand{\inn}{
\newcommand{\SUM}{\displaystyle \sum}
\newcommand{\MAX}{\displaystyle \max}
\newcommand{\MIN}{\displaystyle \min}
\newcommand{\Prob}{\mathsf{P}}

\newcommand{\argmax}[1]{\underset{#1}{\mathrm{argmax}}}
\newcommand{\argmin}[1]{\underset{#1}{\mathrm{argmin}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\floor}[1]{\lfloor#1\rfloor}
\newcommand{\ceil}[1]{\lceil#1\rceil}
\newcommand{\fract}[2]{\textstyle\frac{#1}{#2}}
\newcommand{\sumto}[3]{\sum_{{#1}=#2}^{#3}}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ones}{\mathsf{\mathbf{1}}}
%\newcommand{\inn}[2]{\langle#1,#2\rangle}

%% -------- MATH SYMBOLS ---------------- %%

\newcommand{\Co}{\mbox{conv}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\sign}{\mathrm{sign}}
%\newcommand{\argmin}[1]{\underset{#1}{\mathrm{argmin}}}
\newcommand{\KL}{\mathrm{D}_{\textrm{\tiny KL}}}

\newcommand{\loss}{\ell}
\newcommand{\sumt}{\textstyle\sum}

\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\boldeta}{\boldsymbol{\eta}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bell}{\boldsymbol{\ell}}

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\boldf}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\PD}{\mathcal{S}_{++}^p}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

\newcommand{\bzero}{\boldsymbol{0}}
\newcommand{\bone}{\boldsymbol{1}}

\newcommand{\hs}{h^\star}
\newcommand{\Hs}{H^\star}

\newcommand{\R}{\mathbb{R}}
\newcommand{\Sy}{\mathbb{S}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\secref}[1]{Sec.~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
%\renewcommand{\eqref}[1]{Eq.~(\ref{#1})}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\thmref}[1]{Thm.~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}

\newcommand{\diag}{\mbox{diag}}


%% -------------- SJGL PAPER SPECIFIC MACROS --------------- %%

\newcommand{\thetasymb}{\boldsymbol{\Theta}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bThetaone}{{\boldsymbol{\Theta}}^1}
\newcommand{\bThetatwo}{{\boldsymbol{\Theta}}^2}
\newcommand{\bThetai}{{\boldsymbol{\Theta}}^i}
\newcommand{\bThetaj}{{\boldsymbol{\Theta}}^j}
\newcommand{\bThetak}{{\boldsymbol{\Theta}}^k}
\newcommand{\bThetaK}{{\boldsymbol{\Theta}}^K}
\newcommand{\var}{\boldsymbol{\Theta}}
\newcommand{\varone}{{\boldsymbol{\Theta}}^1}
\newcommand{\vartwo}{\boldsymbol{\Theta}^2}
\newcommand{\varK}{{\boldsymbol{\Theta}}^K}
\newcommand{\vari}{{\boldsymbol{\Theta}}^i}
\newcommand{\varj}{{\boldsymbol{\Theta}}^j}
\newcommand{\vark}{{\boldsymbol{\Theta}}^k}
\newcommand{\hatvarone}{{\hat{\boldsymbol{\Theta}}}^1}
\newcommand{\hatvartwo}{\hat{\boldsymbol{\Theta}}^2}
\newcommand{\Lambdaone}{\Lambda^1}
\newcommand{\Lambdatwo}{\Lambda^2}
\newcommand{\Lambdai}{\Lambda^i}
\newcommand{\LambdaK}{\Lambda^K}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\siginvone}{({\boldsymbol{\Sigma}}^1)^{-1}}
\newcommand{\siginvtwo}{({\boldsymbol{\Sigma}}^2)^{-1}}
\newcommand{\Omegand}{\Omega^{\scriptsize \operatorname{N}}_q}
\newcommand{\Omegac}{\Omega^{\scriptsize \operatorname{C}}_q}
\newcommand{\Zone}{{\bf Z}^1}
\newcommand{\Ztwo}{{\bf Z}^2}
\newcommand{\Zi}{{\bf Z}^i}
\newcommand{\ZK}{{\bf Z}^K}
\newcommand{\Yone}{{\bf Y}^1}
\newcommand{\Ytwo}{{\bf Y}^2}
\newcommand{\Yi}{{\bf Y}^i}
\newcommand{\YK}{{\bf Y}^K}
\newcommand{\Qone}{{\bf Q}^1}
\newcommand{\Qtwo}{{\bf Q}^2}
\newcommand{\Qi}{{\bf Q}^i}
\newcommand{\Cone}{{\bC}^1}
\newcommand{\Ctwo}{{\bC}^2}
\newcommand{\Ci}{{\bf C}^i}
\newcommand{\CK}{{\bC}^K}
\newcommand{\Fone}{{\bf F}^1}
\newcommand{\Ftwo}{{\bf F}^2}
\newcommand{\Fi}{{\bf F}^i}
\newcommand{\Gone}{{\bf G}^1}
\newcommand{\Gtwo}{{\bf G}^2}
\newcommand{\Gi}{{\bf G}^i}
\newcommand{\Sone}{{\bf S}_1}
\newcommand{\Stwo}{{\bf S}_2}
\newcommand{\Sii}{{\bf S}^i}
\newcommand{\Ji}{{\mathcal J}_i}
\newcommand{\Vone}{{\bV}^1}
\newcommand{\Vtwo}{{\bV}^2}
\newcommand{\Vij}{{\bV}^{ij}}
\newcommand{\Vi}{{\bV}^i}
\newcommand{\VK}{{\bV}^K}
\newcommand{\Wone}{{\bW}^1}
\newcommand{\Wtwo}{{\bW}^2}
\newcommand{\Wij}{{\bW}^{ij}}
\newcommand{\Wi}{{\bW}^i}
\newcommand{\Wtij}{{({\bW}^{ij})}^T}
\newcommand{\Fij}{{\bF}^{ij}}
\newcommand{\Gij}{{\bG}^{ij}}
\newcommand{\SON}{\mbox{SON}}
\newcommand{\expand}{\mbox{Expand}}
\newcommand{\ADMM}{\mbox{ADMM }}
\newcommand{\JGLsym}{JGL sym-2 }
\newcommand{\sym}{Symmetric overlap norm }
\newcommand{\argmini}{\displaystyle \mathop{\rm argmin}}
\newcommand{\argmaxi}{\displaystyle \mathop{\rm argmax}}
%\newcommand{\thresh}{\mathcal{S}}
\newcommand{\thresh}{\mathcal{T}}
\newcommand{\scal}{\mathcal{T}}
\newcommand{\Expand}{\mbox{Expand}}


\newcommand{\psd}{\mathbb{S}_{++}^{p}}
\newcommand{\regone}{\lambda_1}
\newcommand{\regtwo}{\lambda_2}
\newcommand{\dg}{{\bf g}^d}
\newcommand{\df}{{f}^d}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\second}{\operatorname{second}}
\newcommand{\average}{\operatorname{avg}}
%\newcommand{\inverse}[1]{(#1)^{-1}}
\newcommand{\inverse}[2]{{\widetilde{#1}}^{#2}}

